Fractonic topological phases from coupled wires

In three dimensions, gapped phases can support "fractonic" quasiparticle excitations, which are either completely immobile or can only move within a low-dimensional submanifold, a peculiar topological phenomenon going beyond the conventional framework of topological quantum field theory. In this work we explore fractonic topological phases using three-dimensional coupled wire constructions, which have proven to be a successful tool to realize and characterize topological phases in two dimensions. We find that both gapped and gapless phases with fractonic excitations can emerge from the models. In the gapped case, we argue that fractonic excitations are mobile along the wire direction, but their mobility in the transverse plane is generally reduced. We show that the excitations in general have infinite-order fusion structure, distinct from previously known gapped fracton models. Like the 2D coupled wire constructions, many models exhibit gapless (or even chiral) surface states, which can be described by infinite-component Luttinger liquids. However, the universality class of the surface theory strongly depends on the surface orientation, thus revealing a new type of bulk-boundary correspondence unique to fracton phases.

==> PRR Draft arxiv/type2.tex <==
\onecolumngrid
\section{Proof that the model Eq. \eqref{eqn:type2} has only lineons}
\label{sec:type2}
Recall that the stabilizer map is given by
\begin{equation}
\sigma=\left(\begin{array}{ccc}
x+y+xy& & \\
n+x+y& & \\
& n+\overline{x}+\overline{y} \\
& -(\overline{x}+\overline{y}+\overline{xy})
\end{array}\right). 
\end{equation}

Formally the stabilizers can be written as
 \begin{align}
 \label{stabtype3}
 \begin{array}{c}
 \plaquette{XX}{XI}{IX^{n}}{XX}
 \quad\quad
 \plaquette{ZZ^{-1}}{Z^nI}{IZ^{-1}}{ZZ^{-1}}
 \end{array}
 \end{align}
 Here for brevity and in analogy with stabilizer codes we denote $XI\equiv e^{i\phi_1}, IX\equiv e^{i\phi_2}, ZI\equiv e^{i\theta_1}, IZ\equiv e^{i\theta_2}$, suppressing the $x$ coordinate dependence.
We consider cleaning of arbitrary pair creation operators to show that there is nontrivial logical string operator. Since the code is ``CSS'', cleaning the pair creation operators of one type would be enough. Thus, we consider $Z$ pair creation operators. 

\subsection{Cleaning to a minimal box containing the excitation patches}
We can clean an arbitrary pair creation operator that creates a pair of excitation patches to a minimal box that contains the two patches. This can be done by using the commutation constraints due to the corners shared with X stabilizers, i.e. where the independent vertices $XI$ and $XX$ of the X stabilizer operator hits the pair creation operator enclosing the excitation patches. There are two orthogonal edges with these type of independent vertices, $XX$ and $XI$, in the X stabilizer. Such edges are called good edges for cleaning~\cite{Haah} and having two of them here implies that one can clean the Z pair creation operator down to a minimal box containing the excitation patches as shown in Figs.~\ref{pc122}, \ref{pc342} and \ref{pc562} using commutation constraints with the corners of the kind $XX$ and $XI$ of the X stabilizer. 

\subsection{Diagonal pair creation operators}
The figures \ref{pc122}(a) and \ref{pc342}(a) can be cleaned to flat-rod configurations by just step-wise cleaning of corners. For example, in  Fig. \ref{pc122}a, use $[O,XX]=0$ which gives $O=ZZ^{-1}$ and thus it can be cleaned by multiplying the Z-stabilizer. The process can be repeated for $O_1$ and $O_2$ and so on to yield Fig.~\ref{pc122}(c). The same process can be carried out for configuration in fig.~\ref{pc342}(a) to yield Fig~\ref{pc342}c using the constraint $[O,XI]=0$ which yields $O=IZ, II$.


\begin{figure}[H]
\vspace{6mm}
\centering
\sidesubfloat[]{\includegraphics[scale=0.28]{pc1.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc1b.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc1c.pdf}}
\caption{Cleaning of pair creation operators}
\label{pc122}
\end{figure}

\begin{figure}[H]
\vspace{6mm}
\centering
\sidesubfloat[]{\includegraphics[scale=0.28]{pc3a.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc3b.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc3c.pdf}}
\caption{Cleaning of pair creation operators}
\label{pc342}
\end{figure}


\subsection{Horizontal and vertical strips}
The horizontal and vertical strips can be reduced again to the lines. For the horizontal line, we can show the deformation result for recursion as follows. Suppose the operator on site $i$ is $(a_i, b_i)$. Then they must satisfy
\begin{equation}
    a_i+b_i+a_{i+1}=0, nb_i + a_{i+1}+b_{i+1}=0.
\end{equation}
It follows that $a_{i+2}=nb_i$, and
\begin{equation}
    n(a_i+a_{i+1})+a_{i+2}=0.
\end{equation}
The characteristic polynomial is $x^2+nx+n=0$, with roots $\omega_{1,2}=\frac{-n\pm \sqrt{n(n-4)}}{2}$. So we can generally write
\begin{equation}
    a_i = u_1\omega_1^i + u_2 \omega_2^i.
\end{equation}
Then
\begin{equation}
    b_i = -a_i-a_{i+1}=-u_1(1+\omega_1)\omega_1^i - u_2(1+\omega_2)\omega_2^i.
\end{equation}
It is easy to see that if $n>4$, both $\omega_{1,2}$ are real and $|\omega_{1,2}|>1$, so $a_i$ or $b_i$ grows exponentially large with $i$.

\begin{figure}[H]
\vspace{6mm}
\centering
\sidesubfloat[]{\includegraphics[scale=0.28]{pc6a.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc6b.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc6c.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc6d.pdf}}\\ \vspace{1cm}

\sidesubfloat[]{\includegraphics[scale=0.28]{pc52a.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc52b.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc52c.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc52d.pdf}}
\caption{Cleaning of pair creation operators}
\label{pc562}
\end{figure}
Similarly, for the vertical line, we have the recursion relations 
\begin{equation}
    a_i+a_{i+1}+b_{i+1}=0, a_i+b_i +n b_{i+1}=0.
\end{equation}
It follows that $a_i=n b_{i+2}$, and
\begin{equation}
   nb_{i+2}+nb_{i+3}+b_{i+1}=0.
\end{equation}
The characteristic polynomial is $nx^2+nx+1=0$, with roots $\lambda_{1,2}=-\frac{1}{2}\pm \sqrt{\frac{1}{4}-\frac{1}{n}}$. So we can generally write
\begin{equation}
        b_i = u_1\lambda_1^i + u_2 \lambda_2^i.
\end{equation}
Then
\begin{equation}
  a_i=-b_i-n b_{i+1}=-u_1(1+n\lambda_1)\lambda_1^i - u_2(1+n\lambda_2) \lambda_2^i.
\end{equation}
When $n\geq 4$, both roots $|\lambda_{1,2}|<1$. As a result, $a_i$ and $b_i$ decays exponentially and the string can not extend to arbitrarily long length. 

We have shown that both horizontal and vertical string operators must create charges exponentially large in the length of the string at least on one end. Now we further prove explicitly that no string operators can create charges of opposite values, meaning $nb_i = -a_0-b_0$ and $a_i+b_i= -a_0$. Consider the horizontal line. This implies 
\begin{equation}
n[u_1(1+\omega_1)\omega_1^i+ u_2(1+\omega_2)\omega_2^i]= u_1(2+\omega_1)+ u_2(2+\omega_2),
\end{equation}
and 
\begin{equation}
    u_1\omega_1^{i+1} + u_2 \omega_2^{i+1}= u_1+u_2.
\end{equation}
They have no non-zero solution for any $i$. Similar holds for the vertical relations. 

\subsection{L shaped operators}

\begin{figure}[H]
\vspace{6mm}
\centering
\sidesubfloat[]{\includegraphics[scale=0.28]{Lshaped.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{Lshapea.pdf}}\\
\vspace{10 mm}
\sidesubfloat[]{\includegraphics[scale=0.28]{Lshapeb.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{Lshapec.pdf}}\\
\caption{L shaped operators}
\label{Lshape}
\end{figure}

We now consider string operators that could be formed from L shaped operators in Fig.~\ref{pc122}(c) and Fig.~\ref{pc342}(c). Using the cleaning done for the horizontal and vertical strips, we can reduce these operators to width 1 operators shown in Fig.~\ref{Lshape}. The lines do not join exactly at the corner in order to cancel out the excitations around it. The patches shown at the ends show the excitation strengths at those ends. We now show string operator formed from such joining L shaped width 1 operators cannot form a nontrivial logical operator.  

\subsubsection{L shaped operators in Fig.~\ref{Lshape}(a) and (b)} 
In Fig.\ref{Lshape}a, due to the commutation with stabilizer generators, the vertices $O_{h0}$ and $O_{v0}$  have constraints $[O_{h0},IX^n]=[O_{v0},IX^n]=0$ which imply $O_{h0}=(ZI)^{n_h}\equiv(n_h,0)$ and $O_{v0}=(ZI)^{n_v}\equiv(n_v,0)$. In order to cancel the excitation shared by the two lines of the L shape as shown, we get $n_h+n_v=0$. Along the horizontal line, we have the recursion constraints due to the commutation as follows
\begin{align}
    a^h_{i+1}+b^h_{i+1}+a_i^h=0\\
    nb^h_{i+1}+a_i^h+b^h_i=0
\end{align}
which give the recursive equation
\begin{equation}
    nb^h_{i+2}+nb^h_{i+1}+b^h_i=0.
\end{equation}
This can be solved using the quadratic $ny^2+ny+1=0$ which has two roots $\lambda_1,\lambda_2$. Thus, we get for the other corner $(a^h_i,b^h_i)$,
\begin{align}
    b_i^h&=u_1^h\lambda_1^i+u_2^h\lambda_2^i\label{solah1}\\
    a_i^h&=-u_1^h(1+n\lambda_1)\lambda_1^i-u_2^h(1+n\lambda_2)\lambda_2^i.\label{solah2}
\end{align}
Using the constraint $O_{h0}\equiv(a^h_0,b^h_0)=(-n_v,0)$, we get $u_1^h=-u_2^h=\frac{-n_v}{n(\lambda_2-\lambda_1)}$. 

Similarly, for the vertical line, we have 
\begin{align}
    a_i^v+a_{i+1}^v+b^v_{i+1}&=0\label{vert1}\\
    a_i^v+b_i^v+nb_{i+1}^v&=0
    \label{vert2}
\end{align}
which gives the recursive equation
\begin{equation}
    nb^v_{i+2}+nb^v_{i+1}+b^v_i=0
\end{equation}
with roots $\lambda_{1,2}$ of the same characteristic equation as before i.e.  $ny^2+ny+1=0$. Hence, we again get
\begin{align}
    b_i^v&=u_1^v\lambda_1^i+u_2^v\lambda_2^i \label{solav1}\\
    a_i^v&=-u_1^v(1+n\lambda_1)\lambda_1^i-u_2^v(1+n\lambda_2)\lambda_2^i\label{solav2}.
\end{align}
Using $O_{v0}\equiv(a^v_0,b^v_0)=(n_v,0)$, we get $u_1^v=-u_2^v=\frac{n_v}{n(\lambda_2-\lambda_1)}$. Now, in order for the L shape to form a string operator, we need to cancel out the excitation created at the two ends. Hence, we require $a_i^v=0$, $a_i^h=0$ and $b_i^v+b_i^h=0$. But 
\begin{align}
    a_i^v=\frac{n_1}{\lambda_2-\lambda_1}(\lambda_1^{i+2}-\lambda_2^{i+2}).
\end{align}
We notice that both $\lambda_{1}$ and $\lambda_2$ are negative with $|\lambda_2|>|\lambda_1|$ and thus $a_i^v=0$ is not possible for $n>4$. 

We can have the same L shape with different boundary operators at the corner for the horizontal and vertical segments, as shown in Fig.\ref{Lshape}b. In this case, in order to cancel the excitations in the plaquettes, we get $O_{h0}=(nn_v,0)$ and $O_{v0}=(n_v,-n_v)$. The recursion relations are the same as the L shape in Fig.\ref{Lshape}a because of the same commutation constraints along the edge. Thus, the solutions are of the form \eqref{solav1} and \eqref{solav2} for the horizontal segment and of the form  \eqref{solav1} and \eqref{solav2} for the vertical segment. Only the boundary conditions are different i.e. $O_{h0}=(a^h_0,b^h_0)=(n_v,0)$ and $O_{v0}=(a^v_0,b^v_0)=(n_v,-n_v)$. 
% $u_1^h+u_2^h=0$ and $-u_1^h(1+n\lambda_1)-u_2^h(1+n\lambda_2)= n_v$ for the horizontal segment and $u_1^v+u_2^v=n_v$ and $-u_1^v(1+n\lambda_1)-u_2^v(1+n\lambda_2)= n_v$. 
Hence the solutions for $u_i^{v}$ are modified to be 
$    u_1^v=\frac{n_v\lambda_2}{\lambda_2-\lambda_1}$ and $
    u_2^v=\frac{-n_v\lambda_1}{\lambda_2-\lambda_1}$. 
% \end{align}
% \begin{align}
%     u_1^h&= \frac{nn_v+n_vw_2^2}{w_1^2-w_2^2}
%     \label{solav1}\\
%     u_2^h&=-n_v-u_1^h=\frac{-n_v(w_1^2+2w_2^2)+nn_v}{w_1^2-w_2^2}
%     \label{solav2}.
% \end{align}
% and
To form a string operator, we require as in Fig.~\ref{Lshape}a, $a_i^v=0$, $a_i^h=0$ and $b_i^v+b_i^h=0$. We have 
\begin{align}
	a_i^v=\frac{n_v\lambda_1\lambda_2}{\lambda_1-\lambda_2}\left[(1+n\lambda_2)\lambda_2^{i-1}-(1+n\lambda_1)\lambda_1^{i-1}\right].
\end{align}
We again notice that both $\lambda_{1}$ and $\lambda_2$ are negative with $|\lambda_2|>|\lambda_1|$, and
so it is impossible to have $a_i^v=0$.

% \begin{equation}
% 	\frac{n\lambda_2+2}{n(\lambda_2-\lambda_1)}=1+\sqrt{1-\frac{4}{n}}<2.
% 	\label{}
% \end{equation}
% Therefore 
% \begin{equation}
% 	\left|\frac{n\lambda_2+2}{n(\lambda_2-\lambda_1)}(\lambda_2^{i+1}-\lambda_1^{i+1}) \right|<2|\lambda_2^{i+1}|.
% 	\label{}
% \end{equation}

% We can similarly check the other L-shaped operator as shown in fig.~\ref{Lshape}b. We now have $[O_{h0},XX]=[O_{v0},XX]=0$ such that $O_{h0}=(ZZ^{-1})^n_h$ and $O_{v0}=(ZZ^{-1})^n_v$. In order to cancel the common excitation, we require $n_h=nn_v$. Thus, $O_h=(ZZ^{-1})^n_h\equiv(nn_v,-nn_v)$ and $O_v=(ZZ^{-1})^n_v\equiv(n_v,-n_v)$. 
% For the vertical line, we now have the same constraints as before, thus we get 
% \begin{align}
%     b_i^v&=u_1^v\lambda_{1,v}^i+u_2^v\lambda_{2,v}^i\\
%     a_i^v&=-u_1^v(1+n\lambda_{1,v})\lambda_{1,v}^i-u_2^v(1+n\lambda_{2,v})\lambda_{2,v}^i.
% \end{align}
% where $\lambda_{1,v},\lambda_{2,v}$ are roots of the characteristic equation $ny^2+ny+1=0$. 
% Using $O_2\equiv(a^v_0,b^v_0)=(n_2,-n_2)$, we get $u_1^v=\frac{n_2\lambda_{2,v}}{\lambda_{1,v}-\lambda_{2,v}}$ and $u_2^v=\frac{-n_2\lambda_{1,v}}{\lambda_{1,v}-\lambda_{2,v}}$. 


\subsubsection{L shaped operators in Fig.~\ref{Lshape}(c) and (d)} 
In Fig. \ref{Lshape}c, we have $[O_{h0},XX]=[O_{v0},XX]=0$ such that $O_{h0}=(ZZ^{-1})^{n_h}$ and $O_{v0}=(ZZ^{-1})^{n_v}$. In order to cancel the common excitation, we require $n_h=nn_v$. Thus, $O_h=(ZZ^{-1})^n_h\equiv(nn_v,-nn_v)$ and $O_v=(ZZ^{-1})^n_v\equiv(n_v,-n_v)$. 
For the vertical line, we have the same constraints as \eqref{vert1} and \eqref{vert2}, thus we get 
\begin{align}
    b_i^v&=u_1^v\lambda_1^i+u_2^v\lambda_2^i\\
    a_i^v&=-u_1^v(1+n\lambda_1)\lambda_1^i-u_2^v(1+n\lambda_2)\lambda_2^i.
\end{align}
with roots $\lambda_{1,2}$ of the same characteristic equation as before i.e. $nx^2+nx+1=0$.
Using $O_2\equiv(a^v_0,b^v_0)=(n_2,-n_2)$, we get $u_1^v=\frac{n_2\lambda_2}{\lambda_1-\lambda_2}$ and $u_2^v=\frac{-n_2\lambda_1}{\lambda_1-\lambda_2}$. For the horizontal line, we get
\begin{align}
    nb_i^h+a_{i+1}^h+b_{i+1}^h &=0\\
    a_i^h+b_i^h+a_{i+1}^h &=0
\end{align}
which leads to $n(a^h_i+a_{i+1}^h)+a_{i+2}^h=0$. This leads to 
\begin{align}
    a_i^h&=u_1^h\omega_1^i+u_2^h\omega_2^i\\
    b_i^h&=n^{-1}(u_1^h\omega_1^{i+2}+u_2^h\omega_2^{i+2}),
\end{align}
where $\omega_1,\omega_2$ are roots of the characteristic equation $x^2+nx+n=0$.
Using $a_0^h=u_1^h+u_2^h=nn_v$ and $b_0^h=-nn_v$, we get $u_1^h=\frac{-nn_v(n+\omega_2^2)}{\omega_1^2-\omega_2^2}$ and $u_2^h=\frac{-nn_v(n+\omega_2^2)}{\omega_1^2-\omega_2^2}$. We get 
\begin{align}
    a_i^h+b_i^h&=\frac{n^2n_v}{\omega_2^2-\omega_1^2}(1+n^{-1}\omega_1^2)(1+n^{-1}\omega_2^2)(\omega_1^i-\omega_2^i).
    \label{hor_L2}
\end{align}
The cancellation of excitations requires $a_i^v+b_i^v=0$, $a_i^v+nb_i^h=0$ and $a_i^h+b_i^h=0$. From \eqref{hor_L2}, we see $a_i^h+b_i^h=0$ is not possible for $n>4$. 

We can have the same L shape with different boundary operators at the corner for the horizontal and vertical segments, as shown in Fig.\ref{Lshape}d. In this case, in order to cancel the excitations in the plaquettes, we get the boundary conditions $O_{h0}=(a^h_0,b^h_0)=(-n_v,n_v)$ and $O_{v0}=(a^v_0,b^v_0)=(n_v,0)$.
% As in Fig.\ref{Lshape}b, only the boundary conditions are different i.e. $O_{h0}=(-n_v,n_v)$ and $O_{v0}=(n_v,0)$. $u_1^h+u_2^h=-n_v$ and $n^{-1}(u_1^h w_1^2+u_2^hw_2^2)= n_v$ for the horizontal segment and $u_1^v+u_2^v=0$ and $-u_1^v(1+n\lambda_1)-u_2^v(1+n\lambda_2)= n_v$. 
Hence the solutions for $u_i^{h/v}$ are modified as follows
\begin{align}
    u_1^h=\frac{nn_v+n_v\omega_2^2}{\omega_1^2-\omega_2^2}\\
    u_2^h=\frac{-n_v \omega_1^2-nn_v}{\omega_1^2-\omega_2^2}
\end{align}
which gives 
\begin{align}
    a_i^h+b_i^h&=u_1^h(1+n^{-1}\omega_1^2)\omega_1^i+u_2^h(1+n^{-1}\omega_2^2)\omega_2^i\\
	&=\frac{n_v}{\omega_1^2-\omega_2^2}
	\left\{[(n+\omega_1^2)+(1+n^{-1}w_1^2)\omega_2^2]\omega_1^i-[(n+\omega_2^2)+(1+n^{-1}\omega_2^2)\omega_1^2]\omega_2^i\right\}\\
	&=\frac{n_v n^2}{\omega_1^2-\omega_2^2}
	\left(\omega_1^i-\omega_2^i\right).
%((n+\omega_1^2)\omega_1^i-(n+w_2^2)w_2^i+(1+n^{-1}w_1^2)w_1^iw_2^2-(1+n^{-1}w_2^2)w_2^iw_1^2)
\end{align}
The condition $a_i^h+b_i^h$ to cancel the excitation at the ends to form a string operator cannot be satisfied for $n>4$. 

 




==> type2.tex <==
\onecolumngrid
\section{Proof that the model Eq. \eqref{eqn:type2} has only lineons}
\label{sec:type2}
Recall that the stabilizer map is given by
\begin{equation}
\sigma=\left(\begin{array}{ccc}
x+y+xy& & \\
n+x+y& & \\
& n+\overline{x}+\overline{y} \\
& -(\overline{x}+\overline{y}+\overline{xy})
\end{array}\right). 
\end{equation}

Formally the stabilizers can be written as
 \begin{align}
 \label{stabtype3}
 \begin{array}{c}
 \plaquette{XX}{XI}{IX^{n}}{XX}
 \quad\quad
 \plaquette{ZZ^{-1}}{Z^nI}{IZ^{-1}}{ZZ^{-1}}
 \end{array}
 \end{align}
 Here for brevity and in analogy with stabilizer codes we denote $XI\equiv e^{i\phi_1}, IX\equiv e^{i\phi_2}, ZI\equiv e^{i\theta_1}, IZ\equiv e^{i\theta_2}$, suppressing the $x$ coordinate dependence.
We consider cleaning of arbitrary pair creation operators to show that there is nontrivial logical string operator. Since the code is ``CSS'', cleaning the pair creation operators of one type would be enough. Thus, we consider $Z$ pair creation operators. 

\subsection{Cleaning to a minimal box containing the excitation patches}
We can clean an arbitrary pair creation operator that creates a pair of excitation patches to a minimal box that contains the two patches. This can be done by using the commutation constraints due to the corners shared with X stabilizers, i.e. where the independent vertices $XI$ and $XX$ of the X stabilizer operator hits the pair creation operator enclosing the excitation patches. There are two orthogonal edges with these type of independent vertices, $XX$ and $XI$, in the X stabilizer. Such edges are called good edges for cleaning~\cite{Haah} and having two of them here implies that one can clean the Z pair creation operator down to a minimal box containing the excitation patches as shown in Figs.~\ref{pc122}, \ref{pc342} and \ref{pc562} using commutation constraints with the corners of the kind $XX$ and $XI$ of the X stabilizer. 

\subsection{Diagonal pair creation operators}
The figures \ref{pc122}(a) and \ref{pc342}(a) can be cleaned to flat-rod configurations by just step-wise cleaning of corners. For example, in  Fig. \ref{pc122}a, use $[O,XX]=0$ which gives $O=ZZ^{-1}$ and thus it can be cleaned by multiplying the Z-stabilizer. The process can be repeated for $O_1$ and $O_2$ and so on to yield Fig.~\ref{pc122}(c). The same process can be carried out for configuration in fig.~\ref{pc342}(a) to yield Fig~\ref{pc342}c using the constraint $[O,XI]=0$ which yields $O=IZ, II$.


\begin{figure}[H]
\vspace{6mm}
\centering
\sidesubfloat[]{\includegraphics[scale=0.28]{pc1.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc1b.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc1c.pdf}}
\caption{Cleaning of pair creation operators}
\label{pc122}
\end{figure}

\begin{figure}[H]
\vspace{6mm}
\centering
\sidesubfloat[]{\includegraphics[scale=0.28]{pc3a.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc3b.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc3c.pdf}}
\caption{Cleaning of pair creation operators}
\label{pc342}
\end{figure}


\subsection{Horizontal and vertical strips}
The horizontal and vertical strips can be reduced again to the lines. For the horizontal line, we can show the deformation result for recursion as follows. Suppose the operator on site $i$ is $(a_i, b_i)$. Then they must satisfy
\begin{equation}
    a_i+b_i+a_{i+1}=0, nb_i + a_{i+1}+b_{i+1}=0.
\end{equation}
It follows that $a_{i+2}=nb_i$, and
\begin{equation}
    n(a_i+a_{i+1})+a_{i+2}=0.
\end{equation}
The characteristic polynomial is $x^2+nx+n=0$, with roots $\omega_{1,2}=\frac{-n\pm \sqrt{n(n-4)}}{2}$. So we can generally write
\begin{equation}
    a_i = u_1\omega_1^i + u_2 \omega_2^i.
\end{equation}
Then
\begin{equation}
    b_i = -a_i-a_{i+1}=-u_1(1+\omega_1)\omega_1^i - u_2(1+\omega_2)\omega_2^i.
\end{equation}
It is easy to see that if $n>4$, both $\omega_{1,2}$ are real and $|\omega_{1,2}|>1$, so $a_i$ or $b_i$ grows exponentially large with $i$.

\begin{figure}[H]
\vspace{6mm}
\centering
\sidesubfloat[]{\includegraphics[scale=0.28]{pc6a.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc6b.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc6c.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc6d.pdf}}\\ \vspace{1cm}

\sidesubfloat[]{\includegraphics[scale=0.28]{pc52a.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc52b.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc52c.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{pc52d.pdf}}
\caption{Cleaning of pair creation operators}
\label{pc562}
\end{figure}
Similarly, for the vertical line, we have the recursion relations 
\begin{equation}
    a_i+a_{i+1}+b_{i+1}=0, a_i+b_i +n b_{i+1}=0.
\end{equation}
It follows that $a_i=n b_{i+2}$, and
\begin{equation}
   nb_{i+2}+nb_{i+3}+b_{i+1}=0.
\end{equation}
The characteristic polynomial is $nx^2+nx+1=0$, with roots $\lambda_{1,2}=-\frac{1}{2}\pm \sqrt{\frac{1}{4}-\frac{1}{n}}$. So we can generally write
\begin{equation}
        b_i = u_1\lambda_1^i + u_2 \lambda_2^i.
\end{equation}
Then
\begin{equation}
  a_i=-b_i-n b_{i+1}=-u_1(1+n\lambda_1)\lambda_1^i - u_2(1+n\lambda_2) \lambda_2^i.
\end{equation}
When $n\geq 4$, both roots $|\lambda_{1,2}|<1$. As a result, $a_i$ and $b_i$ decays exponentially and the string can not extend to arbitrarily long length. 

We have shown that both horizontal and vertical string operators must create charges exponentially large in the length of the string at least on one end. Now we further prove explicitly that no string operators can create charges of opposite values, meaning $nb_i = -a_0-b_0$ and $a_i+b_i= -a_0$. Consider the horizontal line. This implies 
\begin{equation}
n[u_1(1+\omega_1)\omega_1^i+ u_2(1+\omega_2)\omega_2^i]= u_1(2+\omega_1)+ u_2(2+\omega_2),
\end{equation}
and 
\begin{equation}
    u_1\omega_1^{i+1} + u_2 \omega_2^{i+1}= u_1+u_2.
\end{equation}
They have no non-zero solution for any $i$. Similar holds for the vertical relations. 

\subsection{L shaped operators}

\begin{figure}[H]
\vspace{6mm}
\centering
\sidesubfloat[]{\includegraphics[scale=0.28]{Lshaped.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{Lshapea.pdf}}\\
\vspace{10 mm}
\sidesubfloat[]{\includegraphics[scale=0.28]{Lshapeb.pdf}}
\sidesubfloat[]{\includegraphics[scale=0.28]{Lshapec.pdf}}\\
\caption{L shaped operators}
\label{Lshape}
\end{figure}

We now consider string operators that could be formed from L shaped operators in Fig.~\ref{pc122}(c) and Fig.~\ref{pc342}(c). Using the cleaning done for the horizontal and vertical strips, we can reduce these operators to width 1 operators shown in Fig.~\ref{Lshape}. The lines do not join exactly at the corner in order to cancel out the excitations around it. The patches shown at the ends show the excitation strengths at those ends. We now show string operator formed from such joining L shaped width 1 operators cannot form a nontrivial logical operator.  

\subsubsection{L shaped operators in Fig.~\ref{Lshape}(a) and (b)} 
In Fig.\ref{Lshape}a, due to the commutation with stabilizer generators, the vertices $O_{h0}$ and $O_{v0}$  have constraints $[O_{h0},IX^n]=[O_{v0},IX^n]=0$ which imply $O_{h0}=(ZI)^{n_h}\equiv(n_h,0)$ and $O_{v0}=(ZI)^{n_v}\equiv(n_v,0)$. In order to cancel the excitation shared by the two lines of the L shape as shown, we get $n_h+n_v=0$. Along the horizontal line, we have the recursion constraints due to the commutation as follows
\begin{align}
    a^h_{i+1}+b^h_{i+1}+a_i^h=0\\
    nb^h_{i+1}+a_i^h+b^h_i=0
\end{align}
which give the recursive equation
\begin{equation}
    nb^h_{i+2}+nb^h_{i+1}+b^h_i=0.
\end{equation}
This can be solved using the quadratic $ny^2+ny+1=0$ which has two roots $\lambda_1,\lambda_2$. Thus, we get for the other corner $(a^h_i,b^h_i)$,
\begin{align}
    b_i^h&=u_1^h\lambda_1^i+u_2^h\lambda_2^i\label{solah1}\\
    a_i^h&=-u_1^h(1+n\lambda_1)\lambda_1^i-u_2^h(1+n\lambda_2)\lambda_2^i.\label{solah2}
\end{align}
Using the constraint $O_{h0}\equiv(a^h_0,b^h_0)=(-n_v,0)$, we get $u_1^h=-u_2^h=\frac{-n_v}{n(\lambda_2-\lambda_1)}$. 

Similarly, for the vertical line, we have 
\begin{align}
    a_i^v+a_{i+1}^v+b^v_{i+1}&=0\label{vert1}\\
    a_i^v+b_i^v+nb_{i+1}^v&=0
    \label{vert2}
\end{align}
which gives the recursive equation
\begin{equation}
    nb^v_{i+2}+nb^v_{i+1}+b^v_i=0
\end{equation}
with roots $\lambda_{1,2}$ of the same characteristic equation as before i.e.  $ny^2+ny+1=0$. Hence, we again get
\begin{align}
    b_i^v&=u_1^v\lambda_1^i+u_2^v\lambda_2^i \label{solav1}\\
    a_i^v&=-u_1^v(1+n\lambda_1)\lambda_1^i-u_2^v(1+n\lambda_2)\lambda_2^i\label{solav2}.
\end{align}
Using $O_{v0}\equiv(a^v_0,b^v_0)=(n_v,0)$, we get $u_1^v=-u_2^v=\frac{n_v}{n(\lambda_2-\lambda_1)}$. Now, in order for the L shape to form a string operator, we need to cancel out the excitation created at the two ends. Hence, we require $a_i^v=0$, $a_i^h=0$ and $b_i^v+b_i^h=0$. But 
\begin{align}
    a_i^v=\frac{n_1}{\lambda_2-\lambda_1}(\lambda_1^{i+2}-\lambda_2^{i+2}).
\end{align}
We notice that both $\lambda_{1}$ and $\lambda_2$ are negative with $|\lambda_2|>|\lambda_1|$ and thus $a_i^v=0$ is not possible for $n>4$. 

We can have the same L shape with different boundary operators at the corner for the horizontal and vertical segments, as shown in Fig.\ref{Lshape}b. In this case, in order to cancel the excitations in the plaquettes, we get $O_{h0}=(nn_v,0)$ and $O_{v0}=(n_v,-n_v)$. The recursion relations are the same as the L shape in Fig.\ref{Lshape}a because of the same commutation constraints along the edge. Thus, the solutions are of the form \eqref{solav1} and \eqref{solav2} for the horizontal segment and of the form  \eqref{solav1} and \eqref{solav2} for the vertical segment. Only the boundary conditions are different i.e. $O_{h0}=(a^h_0,b^h_0)=(n_v,0)$ and $O_{v0}=(a^v_0,b^v_0)=(n_v,-n_v)$. 
% $u_1^h+u_2^h=0$ and $-u_1^h(1+n\lambda_1)-u_2^h(1+n\lambda_2)= n_v$ for the horizontal segment and $u_1^v+u_2^v=n_v$ and $-u_1^v(1+n\lambda_1)-u_2^v(1+n\lambda_2)= n_v$. 
Hence the solutions for $u_i^{v}$ are modified to be 
$    u_1^v=\frac{n_v\lambda_2}{\lambda_2-\lambda_1}$ and $
    u_2^v=\frac{-n_v\lambda_1}{\lambda_2-\lambda_1}$. 
% \end{align}
% \begin{align}
%     u_1^h&= \frac{nn_v+n_vw_2^2}{w_1^2-w_2^2}
%     \label{solav1}\\
%     u_2^h&=-n_v-u_1^h=\frac{-n_v(w_1^2+2w_2^2)+nn_v}{w_1^2-w_2^2}
%     \label{solav2}.
% \end{align}
% and
To form a string operator, we require as in Fig.~\ref{Lshape}a, $a_i^v=0$, $a_i^h=0$ and $b_i^v+b_i^h=0$. We have 
\begin{align}
	a_i^v=\frac{n_v\lambda_1\lambda_2}{\lambda_1-\lambda_2}\left[(1+n\lambda_2)\lambda_2^{i-1}-(1+n\lambda_1)\lambda_1^{i-1}\right].
\end{align}
We again notice that both $\lambda_{1}$ and $\lambda_2$ are negative with $|\lambda_2|>|\lambda_1|$, and
so it is impossible to have $a_i^v=0$.

% \begin{equation}
% 	\frac{n\lambda_2+2}{n(\lambda_2-\lambda_1)}=1+\sqrt{1-\frac{4}{n}}<2.
% 	\label{}
% \end{equation}
% Therefore 
% \begin{equation}
% 	\left|\frac{n\lambda_2+2}{n(\lambda_2-\lambda_1)}(\lambda_2^{i+1}-\lambda_1^{i+1}) \right|<2|\lambda_2^{i+1}|.
% 	\label{}
% \end{equation}

% We can similarly check the other L-shaped operator as shown in fig.~\ref{Lshape}b. We now have $[O_{h0},XX]=[O_{v0},XX]=0$ such that $O_{h0}=(ZZ^{-1})^n_h$ and $O_{v0}=(ZZ^{-1})^n_v$. In order to cancel the common excitation, we require $n_h=nn_v$. Thus, $O_h=(ZZ^{-1})^n_h\equiv(nn_v,-nn_v)$ and $O_v=(ZZ^{-1})^n_v\equiv(n_v,-n_v)$. 
% For the vertical line, we now have the same constraints as before, thus we get 
% \begin{align}
%     b_i^v&=u_1^v\lambda_{1,v}^i+u_2^v\lambda_{2,v}^i\\
%     a_i^v&=-u_1^v(1+n\lambda_{1,v})\lambda_{1,v}^i-u_2^v(1+n\lambda_{2,v})\lambda_{2,v}^i.
% \end{align}
% where $\lambda_{1,v},\lambda_{2,v}$ are roots of the characteristic equation $ny^2+ny+1=0$. 
% Using $O_2\equiv(a^v_0,b^v_0)=(n_2,-n_2)$, we get $u_1^v=\frac{n_2\lambda_{2,v}}{\lambda_{1,v}-\lambda_{2,v}}$ and $u_2^v=\frac{-n_2\lambda_{1,v}}{\lambda_{1,v}-\lambda_{2,v}}$. 


\subsubsection{L shaped operators in Fig.~\ref{Lshape}(c) and (d)} 
In Fig. \ref{Lshape}c, we have $[O_{h0},XX]=[O_{v0},XX]=0$ such that $O_{h0}=(ZZ^{-1})^{n_h}$ and $O_{v0}=(ZZ^{-1})^{n_v}$. In order to cancel the common excitation, we require $n_h=nn_v$. Thus, $O_h=(ZZ^{-1})^n_h\equiv(nn_v,-nn_v)$ and $O_v=(ZZ^{-1})^n_v\equiv(n_v,-n_v)$. 
For the vertical line, we have the same constraints as \eqref{vert1} and \eqref{vert2}, thus we get 
\begin{align}
    b_i^v&=u_1^v\lambda_1^i+u_2^v\lambda_2^i\\
    a_i^v&=-u_1^v(1+n\lambda_1)\lambda_1^i-u_2^v(1+n\lambda_2)\lambda_2^i.
\end{align}
with roots $\lambda_{1,2}$ of the same characteristic equation as before i.e. $nx^2+nx+1=0$.
Using $O_2\equiv(a^v_0,b^v_0)=(n_2,-n_2)$, we get $u_1^v=\frac{n_2\lambda_2}{\lambda_1-\lambda_2}$ and $u_2^v=\frac{-n_2\lambda_1}{\lambda_1-\lambda_2}$. For the horizontal line, we get
\begin{align}
    nb_i^h+a_{i+1}^h+b_{i+1}^h &=0\\
    a_i^h+b_i^h+a_{i+1}^h &=0
\end{align}
which leads to $n(a^h_i+a_{i+1}^h)+a_{i+2}^h=0$. This leads to 
\begin{align}
    a_i^h&=u_1^h\omega_1^i+u_2^h\omega_2^i\\
    b_i^h&=n^{-1}(u_1^h\omega_1^{i+2}+u_2^h\omega_2^{i+2}),
\end{align}
where $\omega_1,\omega_2$ are roots of the characteristic equation $x^2+nx+n=0$.
Using $a_0^h=u_1^h+u_2^h=nn_v$ and $b_0^h=-nn_v$, we get $u_1^h=\frac{-nn_v(n+\omega_2^2)}{\omega_1^2-\omega_2^2}$ and $u_2^h=\frac{-nn_v(n+\omega_2^2)}{\omega_1^2-\omega_2^2}$. We get 
\begin{align}
    a_i^h+b_i^h&=\frac{n^2n_v}{\omega_2^2-\omega_1^2}(1+n^{-1}\omega_1^2)(1+n^{-1}\omega_2^2)(\omega_1^i-\omega_2^i).
    \label{hor_L2}
\end{align}
The cancellation of excitations requires $a_i^v+b_i^v=0$, $a_i^v+nb_i^h=0$ and $a_i^h+b_i^h=0$. From \eqref{hor_L2}, we see $a_i^h+b_i^h=0$ is not possible for $n>4$. 

We can have the same L shape with different boundary operators at the corner for the horizontal and vertical segments, as shown in Fig.\ref{Lshape}d. In this case, in order to cancel the excitations in the plaquettes, we get the boundary conditions $O_{h0}=(a^h_0,b^h_0)=(-n_v,n_v)$ and $O_{v0}=(a^v_0,b^v_0)=(n_v,0)$.
% As in Fig.\ref{Lshape}b, only the boundary conditions are different i.e. $O_{h0}=(-n_v,n_v)$ and $O_{v0}=(n_v,0)$. $u_1^h+u_2^h=-n_v$ and $n^{-1}(u_1^h w_1^2+u_2^hw_2^2)= n_v$ for the horizontal segment and $u_1^v+u_2^v=0$ and $-u_1^v(1+n\lambda_1)-u_2^v(1+n\lambda_2)= n_v$. 
Hence the solutions for $u_i^{h/v}$ are modified as follows
\begin{align}
    u_1^h=\frac{nn_v+n_v\omega_2^2}{\omega_1^2-\omega_2^2}\\
    u_2^h=\frac{-n_v \omega_1^2-nn_v}{\omega_1^2-\omega_2^2}
\end{align}
which gives 
\begin{align}
    a_i^h+b_i^h&=u_1^h(1+n^{-1}\omega_1^2)\omega_1^i+u_2^h(1+n^{-1}\omega_2^2)\omega_2^i\\
	&=\frac{n_v}{\omega_1^2-\omega_2^2}
	\left\{[(n+\omega_1^2)+(1+n^{-1}w_1^2)\omega_2^2]\omega_1^i-[(n+\omega_2^2)+(1+n^{-1}\omega_2^2)\omega_1^2]\omega_2^i\right\}\\
	&=\frac{n_v n^2}{\omega_1^2-\omega_2^2}
	\left(\omega_1^i-\omega_2^i\right).
%((n+\omega_1^2)\omega_1^i-(n+w_2^2)w_2^i+(1+n^{-1}w_1^2)w_1^iw_2^2-(1+n^{-1}w_2^2)w_2^iw_1^2)
\end{align}
The condition $a_i^h+b_i^h$ to cancel the excitation at the ends to form a string operator cannot be satisfied for $n>4$. 

 



